Large-scale Point Cloud Semantic Segmentation with Superpoint Graphs

We propose a novel deep learning-based framework to tackle the challenge of semantic segmentation of large-scale point clouds of millions of points. We argue that the organization of 3D point clouds can be efficiently captured by a structure called superpoint graph (SPG), derived from a partition of the scanned scene into geometrically homogeneous elements. SPGs offer a compact yet rich representation of contextual relationships between object parts, which is then exploited by a graph convolutional network. Our framework sets a new state of the art for segmenting outdoor LiDAR scans (+11.9 and +8.8 mIoU points for both Semantic3D test sets), as well as indoor scans (+12.4 mIoU points for the S3DIS dataset).

==> table_and_chair.tex <==
%---tabletop-----
\node at (0   ,4  ) [point_table_top]  (table_top1){};
\node at (0.5 ,4  ) [point_table_top]  (table_top2){};
\node at (1   ,4  ) [point_table_top]  (table_top3){}; 
\node at (1.5 ,4  ) [point_table_top]  (table_top4){}; 
\node at (2   ,4  ) [point_table_top]  (table_top5){}; 
\node at (2.5 ,4  ) [point_table_top]  (table_top6){}; 
\node at (3   ,4  ) [point_table_top]  (table_top7){};
\node at (3.5 ,4  ) [point_table_top]  (table_top8){};
\node at (4   ,4  ) [point_table_top]  (table_top9){}; 
\node at (4.5 ,4  ) [point_table_top]  (table_top10){}; 
\node at (5   ,4  ) [point_table_top]  (table_top11){}; 
\node at (5.5 ,4  ) [point_table_top]  (table_top12){}; 
\node at (6   ,4  ) [point_table_top]  (table_top13){};
\node at (6.5 ,4  ) [point_table_top]  (table_top14){};
\node at (7   ,4  ) [point_table_top]  (table_top15){};
%---table_left_leg-----
\node at (1.5 ,0  ) [point_table_left_leg]  (table_left_leg1){};
\node at (1.5 ,0.5) [point_table_left_leg]  (table_left_leg2){};
\node at (1.5 ,1  ) [point_table_left_leg]  (table_left_leg3){}; 
\node at (1.5 ,1.5) [point_table_left_leg]  (table_left_leg4){}; 
\node at (1.5 ,2  ) [point_table_left_leg]  (table_left_leg5){};
\node at (1.5 ,2.5) [point_table_left_leg]  (table_left_leg6){}; 
\node at (1.5 ,3  ) [point_table_left_leg]  (table_left_leg7){};
\node at (1.5 ,3.5) [point_table_left_leg]  (table_left_leg8){}; 
%---table_right_leg-----
\node at (5.5 ,0  ) [point_table_right_leg]  (table_right_leg1){};
\node at (5.5 ,0.5) [point_table_right_leg]  (table_right_leg2){};
\node at (5.5 ,1  ) [point_table_right_leg]  (table_right_leg3){}; 
\node at (5.5 ,1.5) [point_table_right_leg]  (table_right_leg4){}; 
\node at (5.5 ,2  ) [point_table_right_leg]  (table_right_leg5){};
\node at (5.5 ,2.5) [point_table_right_leg]  (table_right_leg6){}; 
\node at (5.5 ,3  ) [point_table_right_leg]  (table_right_leg7){};
\node at (5.5 ,3.5) [point_table_right_leg]  (table_right_leg8){}; 
%---chair_left_leg-----
\node at (6.5 ,0  ) [point_chair_left_leg]  (chair_left_leg1){}; 
\node at (6.5 ,0.5) [point_chair_left_leg]  (chair_left_leg2){};
\node at (6.5 ,1  ) [point_chair_left_leg]  (chair_left_leg3){}; 
\node at (6.5 ,1.5) [point_chair_left_leg]  (chair_left_leg4){};
\node at (6.5 ,2  ) [point_chair_left_leg]  (chair_left_leg5){}; 
%---chair_right_leg-----
\node at (9  ,0  ) [point_chair_right_leg]  (chair_right_leg1){}; 
\node at (9  ,0.5) [point_chair_right_leg]  (chair_right_leg2){};
\node at (9  ,1  ) [point_chair_right_leg]  (chair_right_leg3){}; 
\node at (9  ,1.5) [point_chair_right_leg]  (chair_right_leg4){};
\node at (9  ,2  ) [point_chair_right_leg]  (chair_right_leg5){};
%---chair_seat-----
\node at (6   ,2.5) [point_chair_seat]  (chair_seat1){}; 
\node at (6.5 ,2.5) [point_chair_seat]  (chair_seat2){}; 
\node at (7   ,2.5) [point_chair_seat]  (chair_seat3){}; 
\node at (7.5 ,2.5) [point_chair_seat]  (chair_seat4){};
\node at (8   ,2.5) [point_chair_seat]  (chair_seat5){}; 
\node at (8.5 ,2.5) [point_chair_seat]  (chair_seat6){};
%---chair_back-----
\node at (9  ,2.5) [point_chair_back]  (chair_seat7){};
\node at (9  ,3  ) [point_chair_back]  (chair_back1){}; 
\node at (9  ,3.5) [point_chair_back]  (chair_back2){};
\node at (9  ,4  ) [point_chair_back]  (chair_back3){}; 
\node at (9  ,4.5) [point_chair_back]  (chair_back4){};
\node at (9  ,5  ) [point_chair_back]  (chair_back5){};
\node at (9  ,5.5) [point_chair_back]  (chair_back6){};
\node at (9  ,6  ) [point_chair_back]  (chair_back7){};
